Projected Dynamical Systems on Irregular, Non-Euclidean Domains for Nonlinear Optimization

Continuous-time projected dynamical systems are an elementary class of discontinuous dynamical systems with trajectories that remain in a feasible domain by means of projecting outward-pointing vector fields. They are essential when modeling physical saturation in control systems, constraints of motion, as well as studying projection-based numerical optimization algorithms. Motivated by the emerging application of feedback-based continuous-time optimization schemes that rely on the physical system to enforce nonlinear hard constraints, we study the fundamental properties of these dynamics on general locally-Euclidean sets. Among others, we propose the use of Krasovskii solutions, show their existence on nonconvex, irregular subsets of low-regularity Riemannian manifolds, and investigate how they relate to conventional Carath\'eodory solutions. Furthermore, we establish conditions for uniqueness, thereby introducing a generalized definition of prox-regularity which is suitable for non-flat domains. Finally, we use these results to study the stability and convergence of projected gradient flows as an illustrative application of our framework. We provide simple counter-examples for our main results to illustrate the necessity of our already weak assumptions.

==> Figs/tikz_preamble.tex <==
%\usepackage[utf8]{inputenc}
\usepackage{tikz}

\usepackage{pgfplots}

\usepgfplotslibrary{colorbrewer} 
\usepgfplotslibrary{fillbetween}

% \usepackage{pgfbaselayers}
%\usepgflibrary{arrows}
\usetikzlibrary{arrows.meta}


\usepackage{xcolor}


==> Figs/watershed_diffeo.tex <==

\pgfplotsset{%
	scale only axis,
	width=1.28125in,
	height=1.5in,
	compat=newest,
%	cycle list/Dark2-6
}

\pgfmathsetmacro\s{50}

\pgfmathsetmacro\r{.5}
\pgfmathsetmacro\d{0.2}
\pgfmathsetmacro\vscale{.2}
\pgfmathsetmacro\vsamples{3}

\pgfmathsetmacro\rr{0.53341}
\newcommand{\betaa}[2]{(#2) * (#1)^((#2)-1) /(1 + (#2)^2*(#1)^(2*((#2)-1)))}

\newcommand{\watersheddiffeo}[1]{
  \begin{tikzpicture}		
        \begin{axis}
        [
            set layers=axis on top,
            view={0}{90},
            domain=-0.7:.9,
            domain y=-.75:.75,
            xmin=-.7, xmax=1,
            ticks=none,
            axis lines=middle,
            axis equal,
            axis line style={on layer=axis background},
        ]       

        % unconstrained vector field
        \addplot3[red,quiver={u={1}, v={0}, scale arrows=.2}, -stealth, samples=(2*\vsamples +1), thin, domain=-.7:.7, domain y = -.75:.75, on layer=axis background] {0};   
          
        \ifdim#1pt>0.5pt        	       	
	        
	        % border of feasible set      
	        \addplot[name path=upper, thin, samples=\s]{x^(#1)};    
	        \addplot[name path=lower, thin, samples=\s]{-x^(#1)};
	        \addplot[fill, color=gray!15] fill between[of=upper and lower];
	                  
	        \addplot[name path=upper, thin, samples=\s, domain=0:.05]{x^(#1)};    
	        \addplot[name path=lower, thin, samples=\s, domain=0:.05]{-x^(#1)};    
	        \addplot[fill, color=gray!15] fill between[of=upper and lower];
	         
	        % origin       
	        \draw[red, fill=red] (axis cs: 0,0) circle [radius=0.015];
	        %\node[black, fill=white] at (axis cs: -.05,.9) [left] {$\qquad \alpha = #1$}; 
	        
	        % projected vector fields
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={(1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))},%
					  v={\betaa{t^(1/(#1))}{(#1)}},%
					  scale arrows=\vscale
					}, 
				-stealth, red, thin] 
			({t^(1/#1)}, {t});
			
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={(1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))},%
					  v={-\betaa{t^(1/(#1))}{(#1)}},%
					  scale arrows=\vscale
					}, 
				-stealth, red, thin] 
			({t^(1/#1)}, {-t});            

	        % normal cones
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={(\betaa{t^(1/(#1))}{(#1)})
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%,%
					  v={-(1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%
					  scale arrows=\vscale
					}, 
				-stealth, black, thick] 
			({t^(1/#1)}, {t});
			
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={(\betaa{t^(1/(#1))}{(#1)})
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%,%
					  v={(1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%
					  scale arrows=\vscale
					}, 
				-stealth, black, thick] 
			({t^(1/#1)}, {-t});    
		\else
	        \fill[fill=gray!15] (0, -.85) rectangle (.9, .85);
	         
	        % origin       
	        \draw[red, fill=red] (axis cs: 0,0) circle [radius=0.015];
	        %\node[black, fill=white] at (axis cs: -.05,.9) [left] {$\qquad \alpha = #1$}; 
	        
	        % projected vector fields
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={0},%
					  v={\betaa{t^(1/(#1))}{(#1)}},%
					  scale arrows=\vscale
					}, 
				-stealth, red, thin] 
			({0}, {t});
			
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={0},%
					  v={-\betaa{t^(1/(#1))}{(#1)}},%
					  scale arrows=\vscale
					}, 
				-stealth, red, thin] 
			({0}, {-t});            

	        % normal cones
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={(\betaa{t^(1/(#1))}{(#1)})
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%,%
					  v={-(1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%
					  scale arrows=\vscale
					}, 
				-stealth, black, thick] 
			({0}, {t});
			
	        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
					variable=\t,
					quiver={%
					  u={(\betaa{t^(1/(#1))}{(#1)})
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%,%
					  v={(1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))
					      /((1 - (#1)* \betaa{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))^2 + (\betaa{t^(1/(#1))}{(#1)})^2)^(1/2)},%
					  scale arrows=\vscale
					}, 
				-stealth, black, thick] 
			({0}, {-t});            
        \fi        

        \end{axis}      
  \end{tikzpicture}
}

==> Figs/watershed_pds.tex <==
\pgfplotsset{%
	scale only axis,
	width=1.1in,
	height=1.2in,
	compat=newest,
%	cycle list/Dark2-6
}

\pgfmathsetmacro\s{50}

\pgfmathsetmacro\r{.5}
\pgfmathsetmacro\d{0.2}
\pgfmathsetmacro\vscale{.2}
\pgfmathsetmacro\vsamples{3}

\pgfmathsetmacro\rr{0.53341}
\newcommand{\bet}[2]{(#2) * (#1)^((#2)-1) /(1 + (#2)^2*(#1)^(2*((#2)-1)))}

\newcommand{\watershedpds}[2]{
  \begin{tikzpicture}[thick,scale=(#2), every node/.style={scale=(#2)}]
        \begin{axis}
        [
            set layers=axis on top,
            view={0}{90},
            domain=-0.7:.9,
            domain y=-.75:.75,
            xmin=-.7, xmax=1,
            ticks=none,
            axis lines=middle,
            axis equal,
            axis line style={on layer=axis background},
        ]       

        \begin{pgfonlayer}{axis background}
            \addplot[fill, color=gray!15] (-.7, -.90) rectangle (0.0, .90);
            
            \addplot[name path=ceil1, draw=none, samples=\s, domain=.05:.75]{.90};
            \addplot[name path=floor1, draw=none, samples=\s, domain=.05:.75]{-.90};
            \addplot[name path=upper1, thin, samples=\s, domain=.05:.75]{x^(#1)};    
            \addplot[name path=lower1, thin, samples=\s, domain=.05:.75]{-x^(#1)};

            \addplot[name path=ceil2, draw=none, samples=\s, domain=0:.05]{.90};
            \addplot[name path=floor2, draw=none, samples=\s, domain=0:.05]{-.90};
            \addplot[name path=upper2, thin, samples=\s, domain=0:.05]{x^(#1)};    
            \addplot[name path=lower2, thin, samples=\s, domain=0:.05]{-x^(#1)};              


            \addplot[fill, color=gray!15] fill between[of=ceil1 and upper1];
            \addplot[fill, color=gray!15] fill between[of=lower1 and floor1];   
              
            \addplot[fill, color=gray!15] fill between[of=ceil2 and upper2];
            \addplot[fill, color=gray!15] fill between[of=floor2 and lower2];   
                  
            \addplot3[red,quiver={u={1}, v={0}, scale arrows=.2}, -stealth, samples=(2*\vsamples ), thin, domain=-.7:.55, domain y = -.75:.75] {0};   
        % unconstrained vector field

  
        \end{pgfonlayer}
        
        \addplot3[red,quiver={u={1}, v={0}, scale arrows=.2}, -stealth, samples=(2*\vsamples ), thin, domain=-.7:.55, domain y = -.75:.75] {0};   
            
        \addplot[fill, color=gray!0] fill between[of=upper1 and lower1, on layer=main];
        
        \addplot[fill, color=gray!0] fill between[of=lower2 and upper2, on layer=main];      
        \addplot[name path=upper1, thin, samples=\s, domain=.05:.75]{x^(#1)};    
        \addplot[name path=lower1, thin, samples=\s, domain=.05:.75]{-x^(#1)};
        \addplot[name path=upper2, thin, samples=\s, domain=0:.05]{x^(#1)};    
        \addplot[name path=lower2, thin, samples=\s, domain=0:.05]{-x^(#1)};   

                  % origin       
        \draw[red, fill=red] (axis cs: 0,0) circle [radius=0.015];
        %\node[black, fill=white] at (axis cs: -.05,.9) [left] {$\qquad \alpha = #1$}; 
        
        % projected vector fields
        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
				variable=\t,
				quiver={%
				  u={(1 - (#1)* \bet{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))},%
				  v={\bet{t^(1/(#1))}{(#1)}},%
				  scale arrows=\vscale
				}, 
			-stealth, red, thick] 
		({t^(1/#1)}, {t});
		
        \addplot[samples=\vsamples, domain=(0.75/(\vsamples+1)):.75,
				variable=\t,
				quiver={%
				  u={(1 - (#1)* \bet{t^(1/(#1))}{#1}  * (t^(1/(#1)))^((#1) - 1))},%
				  v={-\bet{t^(1/(#1))}{(#1)}},%
				  scale arrows=\vscale
				}, 
			-stealth, red, thick] 
		({t^(1/#1)}, {-t});            

        \end{axis}      
  \end{tikzpicture}
}
